MOEA/D with Adaptative Number of Weight Vectors

The Multi-Objective Evolutionary Algorithm based on Decomposition (MOEA/D) is a popular algorithm for solving Multi-Objective Problems (MOPs). The main component of MOEA/D is to decompose a MOP into easier sub-problems using a set of weight vectors. The choice of the number of weight vectors significantly impacts the performance of MOEA/D. However, the right choice for this number varies, given different MOPs and search stages. Here we adaptively change the number of vectors by removing unnecessary vectors and adding new ones in empty areas of the objective space. Our MOEA/D variant uses the Consolidation Ratio to decide when to change the number of vectors, and then it decides where to add or remove these weighted vectors. We investigate the effects of this adaptive MOEA/D against MOEA/D with a poorly chosen set of vectors, a MOEA/D with fine-tuned vectors and MOEA/D-AWA on the DTLZ and ZDT benchmark functions. We analyse the algorithms in terms of hypervolume, IGD and entropy performance. Our results show that the proposed method is equivalent to MOEA/D with fine-tuned vectors and superior to MOEA/D with poorly defined vectors. Thus, our adaptive mechanism mitigates problems related to the choice of the number of weight vectors in MOEA/D, increasing the final performance of MOEA/D by filling empty areas of the objective space while avoiding premature stagnation of the search progress.

==> files/best_scenario_abe.tex <==
\begin{landscape}
\begin{table*}
\centering
    \caption{Best scenario - mean and standard deviation for all algorithms.} 
    \label{tab::Best_Scenario}
    \scalebox{0.8}{
    % \resizebox{\textwidth}{!}{%
    
        \begin{tabular}{l|ccc|ccc|ccc}
        % \hline \multicolumn{4}{c}{$\bf{HV}$} \\
        % \hline 
         & \multicolumn{3}{c|}{$\bf{HV}$}& \multicolumn{3}{c|}{$\bf{IGD}$}& \multicolumn{3}{c}{$\bf{Entropy}$} \\ \hline 
         & MOEA/D  & AWA & MOEA/D-AV & MOEA/D  & AWA & MOEA/D-AV & MOEA/D  & AWA & MOEA/D-AV \\ 
        \hline 
        
        DTLZ1 & $9.70e-01{\scriptstyle\pm2.00e-02}$ & \cellcolor[gray]{0.85}$9.80e-01{\scriptstyle\pm0.00e+00}$ & $9.50e-01{\scriptstyle\pm6.00e-02}$ & $5.80e-01{\scriptstyle\pm1.30e-01}$ & $5.80e-01{\scriptstyle\pm1.70e-01}$ & \cellcolor[gray]{0.85}$5.70e-01{\scriptstyle\pm1.90e-01}$ & $1.12e+01{\scriptstyle\pm8.80e-01}$ & \cellcolor[gray]{0.85}$1.14e+01{\scriptstyle\pm7.30e-01}$ & $1.03e+01{\scriptstyle\pm1.15e+00}$ \\ 
        
        DTLZ2 & \cellcolor[gray]{0.85}$4.70e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$4.70e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$4.70e-01{\scriptstyle\pm0.00e+00}$ & $1.00e-02{\scriptstyle\pm0.00e+00}$ & $1.00e-02{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & $1.22e+01{\scriptstyle\pm2.00e-02}$ & \cellcolor[gray]{0.85}$1.23e+01{\scriptstyle\pm3.00e-02}$ & $1.22e+01{\scriptstyle\pm4.00e-02}$\\
        

        DTLZ3 & \cellcolor[gray]{0.85}$4.50e-01{\scriptstyle\pm1.00e-02}$ & \cellcolor[gray]{0.85}$4.50e-01{\scriptstyle\pm1.00e-02}$ & $4.40e-01{\scriptstyle\pm2.00e-02}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm1.00e-02}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & $2.00e-02{\scriptstyle\pm1.00e-02}$ & $1.10e+01{\scriptstyle\pm7.20e-01}$ & \cellcolor[gray]{0.85}$1.12e+01{\scriptstyle\pm5.80e-01}$ & $1.01e+01{\scriptstyle\pm1.28e+00}$ \\ 
        
        DTLZ4 & \cellcolor[gray]{0.85}$4.60e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$4.60e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$4.60e-01{\scriptstyle\pm0.00e+00}$& \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & $1.11e+01{\scriptstyle\pm1.60e-01}$ & \cellcolor[gray]{0.85}$1.11e+01{\scriptstyle\pm1.70e-01}$ & $1.09e+01{\scriptstyle\pm1.10e-01}$ \\ 
        
        DTLZ5 & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$6.98e+00{\scriptstyle\pm3.00e-02}$ & \cellcolor[gray]{0.85}$6.98e+00{\scriptstyle\pm2.00e-02}$ & $6.92e+00{\scriptstyle\pm2.00e-02}$\\ 
        
        DTLZ6 & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & $6.58e+00{\scriptstyle\pm0.00e+00}$ & $6.59e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$6.60e+00{\scriptstyle\pm2.00e-02}$\\ 
        
        DTLZ7 & \cellcolor[gray]{0.85}$2.40e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.40e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.40e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & $1.01e+01{\scriptstyle\pm8.00e-02}$ & $1.01e+01{\scriptstyle\pm1.40e-01}$ & \cellcolor[gray]{0.85}$1.02e+01{\scriptstyle\pm2.50e-01}$ \\ 
        
        ZDT1 & $6.60e-01{\scriptstyle\pm0.00e+00}$ & $6.60e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$6.70e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$& \cellcolor[gray]{0.85}$7.26e+00{\scriptstyle\pm3.00e-02}$ & $7.25e+00{\scriptstyle\pm3.00e-02}$ & $7.12e+00{\scriptstyle\pm2.20e-01}$ \\ 
        
        ZDT2 & \cellcolor[gray]{0.85}$3.30e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$3.30e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$3.30e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$  & $7.24e+00{\scriptstyle\pm4.00e-02}$ & \cellcolor[gray]{0.85}$7.25e+00{\scriptstyle\pm9.00e-02}$ & $7.18e+00{\scriptstyle\pm1.70e-01}$ \\ 
        
        
        ZDT3 & \cellcolor[gray]{0.85}$1.04e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.04e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.04e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$6.66e+00{\scriptstyle\pm6.00e-02}$ & $6.65e+00{\scriptstyle\pm5.00e-02}$ & $6.56e+00{\scriptstyle\pm5.00e-01}$ \\ 
        
        ZDT4 & \cellcolor[gray]{0.85}$6.60e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$6.60e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$6.60e-01{\scriptstyle\pm0.00e+00}$& \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$  & $7.20e+00{\scriptstyle\pm6.00e-02}$ & $7.26e+00{\scriptstyle\pm2.00e-02}$ & \cellcolor[gray]{0.85}$7.27e+00{\scriptstyle\pm8.00e-02}$  \\ 
        
        
        ZDT6 & \cellcolor[gray]{0.85}$3.30e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$3.30e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$3.30e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & $6.62e+00{\scriptstyle\pm2.40e-01}$ & \cellcolor[gray]{0.85}$6.71e+00{\scriptstyle\pm2.90e-01}$ & $4.30e+00{\scriptstyle\pm3.70e-01}$ \\ 
        
    \hline
    \hline
        Stats & $=$ & $=$ & & $=$ & $=$ &  & $-$ & $-$ &  \\ 
    % \hline
    % \hline

        \end{tabular}%
        
    }
\end{table*}

\end{landscape}

==> files/best_scenario_abe_mean_only.tex <==
\begin{table*}[htbp]
\centering
    \caption{Best scenario - mean for all algorithms.} 
    \label{tab::Best_Scenario}
    %\scalebox{1}{
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|ccc|ccc|ccc}
        % \hline \multicolumn{4}{c}{$\bf{HV}$} \\
        % \hline 
         & \multicolumn{3}{c|}{$\bf{HV}$}& \multicolumn{3}{c|}{$\bf{IGD}$}& \multicolumn{3}{c}{$\bf{Entropy}$} \\ \hline
         & MOEA/D  & AWA & \textbf{MOEA/D-AV} & MOEA/D  & AWA & \textbf{MOEA/D-AV} & MOEA/D  & AWA & \textbf{MOEA/D-AV} \\ 
        \hline 
        
        DTLZ1 & $9.70e-01$ & \cellcolor[gray]{0.85}$9.80e-01$ & $9.50e-01$ & $5.80e-01$ & $5.80e-01$ & \cellcolor[gray]{0.85}$5.70e-01$ & $1.12e+01$ & \cellcolor[gray]{0.85}$1.14e+01$ & $1.03e+01$ \\ 
        
        DTLZ2 & \cellcolor[gray]{0.85}$4.70e-01$ & \cellcolor[gray]{0.85}$4.70e-01$ & \cellcolor[gray]{0.85}$4.70e-01$ & $1.00e-02$ & $1.00e-02$ & \cellcolor[gray]{0.85}$0.00e+00$ & $1.22e+01$ & \cellcolor[gray]{0.85}$1.23e+01$ & $1.22e+01$\\
        

        DTLZ3 & \cellcolor[gray]{0.85}$4.50e-01$ & \cellcolor[gray]{0.85}$4.50e-01$ & $4.40e-01$ & \cellcolor[gray]{0.85}$1.00e-02$ & \cellcolor[gray]{0.85}$1.00e-02$ & $2.00e-02$ & $1.10e+01$ & \cellcolor[gray]{0.85}$1.12e+01$ & $1.01e+01$ \\ 
        
        DTLZ4 & \cellcolor[gray]{0.85}$4.60e-01$ & \cellcolor[gray]{0.85}$4.60e-01$ & \cellcolor[gray]{0.85}$4.60e-01$& \cellcolor[gray]{0.85}$1.00e-02$ & \cellcolor[gray]{0.85}$1.00e-02$ & \cellcolor[gray]{0.85}$1.00e-02$ & $1.11e+01$ & \cellcolor[gray]{0.85}$1.11e+01$ & $1.09e+01$ \\ 
        
        DTLZ5 & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$6.98e+00$ & \cellcolor[gray]{0.85}$6.98e+00$ & $6.92e+00$\\ 
        
        DTLZ6 & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & $6.58e+00$ & $6.59e+00$ & \cellcolor[gray]{0.85}$6.60e+00$\\ 
        
        DTLZ7 & \cellcolor[gray]{0.85}$2.40e-01$ & \cellcolor[gray]{0.85}$2.40e-01$ & \cellcolor[gray]{0.85}$2.40e-01$ & \cellcolor[gray]{0.85}$1.00e-02$ & \cellcolor[gray]{0.85}$1.00e-02$ & \cellcolor[gray]{0.85}$1.00e-02$ & $1.01e+01$ & $1.01e+01$ & \cellcolor[gray]{0.85}$1.02e+01$ \\ 
        
        ZDT1 & $6.60e-01$ & $6.60e-01$ & \cellcolor[gray]{0.85}$6.70e-01$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$& \cellcolor[gray]{0.85}$7.26e+00$ & $7.25e+00$ & $7.12e+00$ \\ 
        
        ZDT2 & \cellcolor[gray]{0.85}$3.30e-01$ & \cellcolor[gray]{0.85}$3.30e-01$ & \cellcolor[gray]{0.85}$3.30e-01$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$  & $7.24e+00$ & \cellcolor[gray]{0.85}$7.25e+00$ & $7.18e+00$ \\ 
        
        
        ZDT3 & \cellcolor[gray]{0.85}$1.04e+00$ & \cellcolor[gray]{0.85}$1.04e+00$ & \cellcolor[gray]{0.85}$1.04e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$6.66e+00$ & $6.65e+00$ & $6.56e+00$ \\ 
        
        ZDT4 & \cellcolor[gray]{0.85}$6.60e-01$ & \cellcolor[gray]{0.85}$6.60e-01$ & \cellcolor[gray]{0.85}$6.60e-01$& \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$  & $7.20e+00$ & $7.26e+00$ & \cellcolor[gray]{0.85}$7.27e+00$  \\ 
        
        
        ZDT6 & \cellcolor[gray]{0.85}$3.30e-01$ & \cellcolor[gray]{0.85}$3.30e-01$ & \cellcolor[gray]{0.85}$3.30e-01$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & $6.62e+00$ & \cellcolor[gray]{0.85}$6.71e+00$ & $4.30e+00$ \\ 
        
    % \hline
    \hline
        Stats & $=$ & $=$ & & $=$ & $=$ &  & $-$ & $-$ &  \\ 
    % \hline
    % \hline

        \end{tabular}%
    }
\end{table*}

==> files/parameters.tex <==
% \vspace{-2em}
\begin{table}
\begin{center}
\caption{Experimental Parameter Settings}
\label{tab::experimental settings}

\begin{tabular}{cc}
\hline
\textbf{Parameter} & \textbf{Value} \\
\hline
    DE mutation & $ F = 0.5$\\
    Polynomial mutation & $ p_{m} = \frac{1}{N}$\\
    Mating probability & $\delta = 0.9$\\
    Distribution index & $\eta = 20$\\
    Locality parameter & $\delta_p = 0.9$ \\ 
    Neighborhood size & $max(2, \frac{\textnormal{number of vectors}}{10})$ \\
    \hline
    Generation gap ($\Delta$) &$10$\\
    User-controlled fraction (F) & $10$\\
    \hline
    Vector adaption ratio & $0.03$\\
    \hline
    Number of evaluations & $75000$\\
    Trials & $21$\\

\end{tabular}
\end{center}
\end{table}
% \vspace{-1.5em}

==> files/worst_scenario.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Worst Setting Scenario - mean and standard deviation for all algorithms.}
    \label{tab::Worst_Scenario}
    \scalebox{1}{
    \begin{tabular}{l|ccc}
    % \hline \multicolumn{4}{c}{$\bf{HV}$} \\
    \hline $\bf{HV}$ & MOEA/D  & AWA & MOEA/D-AV \\  \hline 
    
DTLZ1 & 0.21 (0.27) & 0.25 (0.33) & \cellcolor[gray]{0.85}0.51 (0.42) \\ 
DTLZ2 & 0.45 (0.00) & 0.45 (0.00) & \cellcolor[gray]{0.85}0.47 (0.00) \\ 
DTLZ3 & 0.01 (0.03) & 0.02 (0.04) & \cellcolor[gray]{0.85}0.15 (0.16) \\ 
DTLZ4 & 0.33 (0.12) & 0.33 (0.15) & \cellcolor[gray]{0.85}0.44 (0.05) \\ 
DTLZ5 & \cellcolor[gray]{0.85}0.22 (0.00) & \cellcolor[gray]{0.85}0.22 (0.00) & \cellcolor[gray]{0.85}0.22 (0.00) \\ 
DTLZ6 & 0.19 (0.08) & \cellcolor[gray]{0.85}0.22 (0.00) & \cellcolor[gray]{0.85}0.22 (0.00) \\ 
DTLZ7 & 0.13 (0.03) & 0.21 (0.03) & \cellcolor[gray]{0.85}0.22 (0.04) \\ 
ZDT1 & 0.03 (0.03) & 0.03 (0.02) & \cellcolor[gray]{0.85}0.12 (0.05) \\ 
ZDT2 & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) \\ 
ZDT3 & 0.20 (0.05) & 0.23 (0.04) & \cellcolor[gray]{0.85}0.33 (0.05) \\ 
ZDT4 & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) \\ 
ZDT6 & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) \\ 
\hline \hline Stats & $+$ & $+$ &  \\ 
% \hline \multicolumn{4}{c}{$\bf{IGD}$} \\
\hline \hline $\bf{IGD}$ & MOEA/D  & AWA & MOEA/D-AV \\ \hline  
DTLZ1 & 1.33 (0.92) & 4.38 (6.26) & \cellcolor[gray]{0.85}0.96 (1.05) \\ 
DTLZ2 & \cellcolor[gray]{0.85}0.01 (0.00) & \cellcolor[gray]{0.85}0.01 (0.00) & \cellcolor[gray]{0.85}0.01 (0.00) \\ 
DTLZ3 & 4.98 (5.45) & 6.96 (7.86) & \cellcolor[gray]{0.85}2.14 (2.85) \\ 
DTLZ4 & 0.33 (0.31) & 0.29 (0.34) & \cellcolor[gray]{0.85}0.06 (0.16) \\ 
DTLZ5 & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) \\ 
DTLZ6 & 0.14 (0.34) & \cellcolor[gray]{0.85}0.00 (0.00) & \cellcolor[gray]{0.85}0.00 (0.00) \\ 
DTLZ7 & 0.39 (0.17) & \cellcolor[gray]{0.85}0.13 (0.17) & 0.15 (0.27) \\ 
ZDT1 & 0.73 (0.13) & 0.69 (0.07) & \cellcolor[gray]{0.85}0.50 (0.09) \\ 
ZDT2 & 1.29 (0.14) & 1.18 (0.19) & \cellcolor[gray]{0.85}0.91 (0.18) \\ 
ZDT3 & 0.61 (0.08) & 0.57 (0.06) & \cellcolor[gray]{0.85}0.46 (0.05) \\ 
ZDT4 & 21.1 (4.34) & 20.5 (4.33) & \cellcolor[gray]{0.85}17.5 (3.16) \\ 
ZDT6 & 5.64 (0.27) & 5.55 (0.36) & \cellcolor[gray]{0.85}5.02 (0.51) \\ 
\hline \hline Stats & $+$ & $+$ &  \\ 
% \hline \hline \multicolumn{4}{c}{$\bf{Entropy}$} \\
\hline \hline \textbf{Entropy} & MOEA/D & AWA & MOEA/D-AV \\ \hline DTLZ1 & 3.75 (0.45) & 3.74 (0.59) & \cellcolor[gray]{0.85} 7.28 (2.04) \\ 
DTLZ2 & 9.19 (0.16) & 8.62 (0.45) & \cellcolor[gray]{0.85} 11.1 (0.31) \\ 
DTLZ3 & 2.67 (0.48) & 1.83 (0.88) & \cellcolor[gray]{0.85} 5.08 (2.58) \\ 
DTLZ4 & 6.00 (1.49) & 5.47 (2.35) & \cellcolor[gray]{0.85} 8.32 (0.84) \\ 
DTLZ5 & 6.45 (0.05) & 5.71 (0.24) & \cellcolor[gray]{0.85}6.66 (0.03) \\ 
DTLZ6 & \cellcolor[gray]{0.85} 6.44 (0.31) & 5.29 (0.24) & 6.17 (0.08) \\ 
DTLZ7 & 8.79 (0.91) & 8.04 (0.70) & \cellcolor[gray]{0.85} 9.22 (0.44) \\ 
ZDT1 & 6.02 (0.27) & 5.91 (0.28) & \cellcolor[gray]{0.85}6.19 (0.20) \\ 
ZDT2 & 2.04 (1.50) & 2.45 (1.47) & \cellcolor[gray]{0.85} 3.38 (1.41) \\ 
ZDT3 & 5.96 (1.60) & 6.02 (0.18) & \cellcolor[gray]{0.85} 6.11 (0.11) \\ 
ZDT4 & 2.67 (0.54) & 6.78 (0.44) & \cellcolor[gray]{0.85} 6.98 (0.25) \\ 
ZDT6 & 3.93 (0.47) & \cellcolor[gray]{0.85} 4.09 (0.61) & 2.64 (1.07) \\ 
\hline \hline Stats & $+$ & $+$ &  \\ \hline \hline
    \end{tabular}
    }
\end{table*}

==> files/worst_scenario_abe.tex <==
\begin{table*}[htbp]
\centering
    \caption{Worst Setting Scenario - mean and standard deviation for all algorithms.} 
    \label{tab::Worst_Scenario}
    %\scalebox{1}{
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|ccc|ccc|ccc}
        % \hline \multicolumn{4}{c}{$\bf{HV}$} \\
        \hline 
         & \multicolumn{3}{c|}{$\bf{HV}$}& \multicolumn{3}{c|}{$\bf{IGD}$}& \multicolumn{3}{c}{$\bf{Entropy}$} \\
         & MOEA/D  & AWA & MOEA/D-AV & MOEA/D  & AWA & MOEA/D-AV & MOEA/D  & AWA & MOEA/D-AV \\ 
        \hline 
        
        DTLZ1 & $2.10e-01{\scriptstyle\pm2.70e-01}$ & $2.50e-01{\scriptstyle\pm3.30e-01}$ & \cellcolor[gray]{0.85}$5.10e-01{\scriptstyle\pm4.20e-01}$ & $1.33e+00{\scriptstyle\pm9.20e-01}$ & $4.38e+00{\scriptstyle\pm6.26e+00}$ & \cellcolor[gray]{0.85}$9.60e-01{\scriptstyle\pm1.05e+00}$  & $3.75e+00{\scriptstyle\pm4.50e-01}$ & $3.74e+00{\scriptstyle\pm5.90e-01}$ & \cellcolor[gray]{0.85}$7.28e+00{\scriptstyle\pm2.04e+00}$  \\ 
        
        DTLZ2& $4.50e-01{\scriptstyle\pm0.00e+00}$ & $4.50e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$4.70e-01{\scriptstyle\pm0.00e+00}$& \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$1.00e-02{\scriptstyle\pm0.00e+00}$  & $9.19e+00{\scriptstyle\pm1.60e-01}$ & $8.62e+00{\scriptstyle\pm4.50e-01}$ & \cellcolor[gray]{0.85}$1.11e+01{\scriptstyle\pm3.10e-01}$ \\
        

        DTLZ3 & $1.00e-02{\scriptstyle\pm3.00e-02}$ & $2.00e-02{\scriptstyle\pm4.00e-02}$ & \cellcolor[gray]{0.85}$1.50e-01{\scriptstyle\pm1.60e-01}$& $4.98e+00{\scriptstyle\pm5.45e+00}$ & $6.96e+00{\scriptstyle\pm7.86e+00}$ & \cellcolor[gray]{0.85}$2.14e+00{\scriptstyle\pm2.85e+00}$& $2.67e+00{\scriptstyle\pm4.80e-01}$ & $1.83e+00{\scriptstyle\pm8.80e-01}$ & \cellcolor[gray]{0.85}$5.08e+00{\scriptstyle\pm2.58e+00}$  \\ 
        
        DTLZ4 & $3.30e-01{\scriptstyle\pm1.20e-01}$ & $3.30e-01{\scriptstyle\pm1.50e-01}$ & \cellcolor[gray]{0.85}$4.40e-01{\scriptstyle\pm5.00e-02}$ & $3.30e-01{\scriptstyle\pm3.10e-01}$ & $2.90e-01{\scriptstyle\pm3.40e-01}$ & \cellcolor[gray]{0.85}$6.00e-02{\scriptstyle\pm1.60e-01}$& $6.00e+00{\scriptstyle\pm1.49e+00}$ & $5.47e+00{\scriptstyle\pm2.35e+00}$ & \cellcolor[gray]{0.85}$8.32e+00{\scriptstyle\pm8.40e-01}$ \\ 
        
        DTLZ5 & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & $6.45e+00{\scriptstyle\pm5.00e-02}$ & $5.71e+00{\scriptstyle\pm2.40e-01}$ & \cellcolor[gray]{0.85}$6.66e+00{\scriptstyle\pm3.00e-02}$ \\ 
        
        DTLZ6  & $1.90e-01{\scriptstyle\pm8.00e-02}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm0.00e+00}$ & $1.40e-01{\scriptstyle\pm3.40e-01}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$6.44e+00{\scriptstyle\pm3.10e-01}$ & $5.29e+00{\scriptstyle\pm2.40e-01}$ & $6.17e+00{\scriptstyle\pm8.00e-02}$\\ 
        
        DTLZ7 & $1.30e-01{\scriptstyle\pm3.00e-02}$ & $2.10e-01{\scriptstyle\pm3.00e-02}$ & \cellcolor[gray]{0.85}$2.20e-01{\scriptstyle\pm4.00e-02}$  & $3.90e-01{\scriptstyle\pm1.70e-01}$ & \cellcolor[gray]{0.85}$1.30e-01{\scriptstyle\pm1.70e-01}$ & $1.50e-01{\scriptstyle\pm2.70e-01}$  & $8.79e+00{\scriptstyle\pm9.10e-01}$ & $8.04e+00{\scriptstyle\pm7.00e-01}$ & \cellcolor[gray]{0.85}$9.22e+00{\scriptstyle\pm4.40e-01}$\\ 
        
        ZDT1  & $3.00e-02{\scriptstyle\pm3.00e-02}$ & $3.00e-02{\scriptstyle\pm2.00e-02}$ & \cellcolor[gray]{0.85}$1.20e-01{\scriptstyle\pm5.00e-02}$& $7.30e-01{\scriptstyle\pm1.30e-01}$ & $6.90e-01{\scriptstyle\pm7.00e-02}$ & \cellcolor[gray]{0.85}$5.00e-01{\scriptstyle\pm9.00e-02}$  & $6.02e+00{\scriptstyle\pm2.70e-01}$ & $5.91e+00{\scriptstyle\pm2.80e-01}$ & \cellcolor[gray]{0.85}$6.19e+00{\scriptstyle\pm2.00e-01}$\\ 
        
        ZDT2 & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & $1.29e+00{\scriptstyle\pm1.40e-01}$ & $1.18e+00{\scriptstyle\pm1.90e-01}$ & \cellcolor[gray]{0.85}$9.10e-01{\scriptstyle\pm1.80e-01}$& $2.04e+00{\scriptstyle\pm1.50e+00}$ & $2.45e+00{\scriptstyle\pm1.47e+00}$ & \cellcolor[gray]{0.85}$3.38e+00{\scriptstyle\pm1.41e+00}$ \\ 
        
        
        ZDT3 & $2.00e-01{\scriptstyle\pm5.00e-02}$ & $2.30e-01{\scriptstyle\pm4.00e-02}$ & \cellcolor[gray]{0.85}$3.30e-01{\scriptstyle\pm5.00e-02}$ & $6.10e-01{\scriptstyle\pm8.00e-02}$ & $5.70e-01{\scriptstyle\pm6.00e-02}$ & \cellcolor[gray]{0.85}$4.60e-01{\scriptstyle\pm5.00e-02}$& $5.96e+00{\scriptstyle\pm1.60e-01}$ & $6.02e+00{\scriptstyle\pm1.80e-01}$ & \cellcolor[gray]{0.85}$6.11e+00{\scriptstyle\pm1.10e-01}$ \\ 
        
        ZDT4 & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & $2.11e+01{\scriptstyle\pm4.34e+00}$ & $2.05e+01{\scriptstyle\pm4.33e+00}$ & \cellcolor[gray]{0.85}$1.75e+01{\scriptstyle\pm3.16e+00}$  & $2.67e+00{\scriptstyle\pm5.40e-01}$ & $6.78e+00{\scriptstyle\pm4.40e-01}$ & \cellcolor[gray]{0.85}$6.98e+00{\scriptstyle\pm2.50e-01}$\\ 
        
        
        ZDT6 & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$ & \cellcolor[gray]{0.85}$0.00e+00{\scriptstyle\pm0.00e+00}$  & $5.64e+00{\scriptstyle\pm2.70e-01}$ & $5.55e+00{\scriptstyle\pm3.60e-01}$ & \cellcolor[gray]{0.85}$5.02e+00{\scriptstyle\pm5.10e-01}$ & $3.93e+00{\scriptstyle\pm4.70e-01}$ & \cellcolor[gray]{0.85}$4.09e+00{\scriptstyle\pm6.10e-01}$ & $2.64e+00{\scriptstyle\pm1.07e+00}$ \\ 
        
    \hline
    \hline
        Stats & $+$ & $+$ & & $+$ & $+$ &  & $+$ & $+$ &  \\ 
    \hline
    \hline

        \end{tabular}%
    }
\end{table*}

==> files/worst_scenario_abe_mean_only.tex <==
\begin{table*}[htbp]
\centering
    \caption{Worst Setting Scenario - mean values for all algorithms.} 
    \label{tab::Worst_Scenario}
    %\scalebox{1}{
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{l|ccc|ccc|ccc}
        % \hline \multicolumn{4}{c}{$\bf{HV}$} \\
        % \hline 
         & \multicolumn{3}{c|}{$\bf{HV}$}& \multicolumn{3}{c|}{$\bf{IGD}$}& \multicolumn{3}{c}{$\bf{Entropy}$} \\ \hline
         & MOEA/D  & AWA & \textbf{MOEA/D-AV} & MOEA/D  & AWA & \textbf{MOEA/D-AV} & MOEA/D  & AWA & \textbf{MOEA/D-AV} \\ 
        \hline 
        
        DTLZ1 & $2.10e-01$ & $2.50e-01$ & \cellcolor[gray]{0.85}$5.10e-01$ & $1.33e+00$ & $4.38e+00$ & \cellcolor[gray]{0.85}$9.60e-01$  & $3.75e+00$ & $3.74e+00$ & \cellcolor[gray]{0.85}$7.28e+00$  \\ 
        
        DTLZ2& $4.50e-01$ & $4.50e-01$ & \cellcolor[gray]{0.85}$4.70e-01$& \cellcolor[gray]{0.85}$1.00e-02$ & \cellcolor[gray]{0.85}$1.00e-02$ & \cellcolor[gray]{0.85}$1.00e-02$  & $9.19e+00$ & $8.62e+00$ & \cellcolor[gray]{0.85}$1.11e+01$ \\
        

        DTLZ3 & $1.00e-02$ & $2.00e-02$ & \cellcolor[gray]{0.85}$1.50e-01$& $4.98e+00$ & $6.96e+00$ & \cellcolor[gray]{0.85}$2.14e+00$& $2.67e+00$ & $1.83e+00$ & \cellcolor[gray]{0.85}$5.08e+00$  \\ 
        
        DTLZ4 & $3.30e-01$ & $3.30e-01$ & \cellcolor[gray]{0.85}$4.40e-01$ & $3.30e-01$ & $2.90e-01$ & \cellcolor[gray]{0.85}$6.00e-02$& $6.00e+00$ & $5.47e+00$ & \cellcolor[gray]{0.85}$8.32e+00$ \\ 
        
        DTLZ5 & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & $6.45e+00$ & $5.71e+00$ & \cellcolor[gray]{0.85}$6.66e+00$ \\ 
        
        DTLZ6  & $1.90e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & \cellcolor[gray]{0.85}$2.20e-01$ & $1.40e-01$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$6.44e+00$ & $5.29e+00$ & $6.17e+00$\\ 
        
        DTLZ7 & $1.30e-01$ & $2.10e-01$ & \cellcolor[gray]{0.85}$2.20e-01$  & $3.90e-01$ & \cellcolor[gray]{0.85}$1.30e-01$ & $1.50e-01$  & $8.79e+00$ & $8.04e+00$ & \cellcolor[gray]{0.85}$9.22e+00$\\ 
        
        ZDT1  & $3.00e-02$ & $3.00e-02$ & \cellcolor[gray]{0.85}$1.20e-01$& $7.30e-01$ & $6.90e-01$ & \cellcolor[gray]{0.85}$5.00e-01$  & $6.02e+00$ & $5.91e+00$ & \cellcolor[gray]{0.85}$6.19e+00$\\ 
        
        ZDT2 & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & $1.29e+00$ & $1.18e+00$ & \cellcolor[gray]{0.85}$9.10e-01$& $2.04e+00$ & $2.45e+00$ & \cellcolor[gray]{0.85}$3.38e+00$ \\ 
        
        
        ZDT3 & $2.00e-01$ & $2.30e-01$ & \cellcolor[gray]{0.85}$3.30e-01$ & $6.10e-01$ & $5.70e-01$ & \cellcolor[gray]{0.85}$4.60e-01$& $5.96e+00$ & $6.02e+00$ & \cellcolor[gray]{0.85}$6.11e+00$ \\ 
        
        ZDT4 & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & $2.11e+01$ & $2.05e+01$ & \cellcolor[gray]{0.85}$1.75e+01$  & $2.67e+00$ & $6.78e+00$ & \cellcolor[gray]{0.85}$6.98e+00$\\ 
        
        
        ZDT6 & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$ & \cellcolor[gray]{0.85}$0.00e+00$  & $5.64e+00$ & $5.55e+00$ & \cellcolor[gray]{0.85}$5.02e+00$ & $3.93e+00$ & \cellcolor[gray]{0.85}$4.09e+00$ & $2.64e+00$ \\ 
        
    % \hline
    \hline
        Stats & $+$ & $+$ & & $+$ & $+$ &  & $+$ & $+$ &  \\ 
    % \hline
    % \hline

        \end{tabular}%
    }
\end{table*}
